ACNPU: A 4.75TOPS/W 1080P@30FPS Super Resolution Accelerator with Decoupled Asymmetric Convolution

Deep learning-driven superresolution (SR) outperforms traditional techniques but also faces the challenge of high complexity and memory bandwidth. This challenge leads many accelerators to opt for simpler and shallow models like FSRCNN, compromising performance for real-time needs, especially for resource-limited edge devices. This paper proposes an energy-efficient SR accelerator, ACNPU, to tackle this challenge. The ACNPU enhances image quality by 0.34dB with a 27-layer model, but needs 36\% less complexity than FSRCNN, while maintaining a similar model size, with the \textit{decoupled asymmetric convolution and split-bypass structure}. The hardware-friendly 17K-parameter model enables \textit{holistic model fusion} instead of localized layer fusion to remove external DRAM access of intermediate feature maps. The on-chip memory bandwidth is further reduced with the \textit{input stationary flow} and \textit{parallel-layer execution} to reduce power consumption. Hardware is regular and easy to control to support different layers by \textit{processing elements (PEs) clusters with reconfigurable input and uniform data flow}. The implementation in the 40 nm CMOS process consumes 2333 K gate counts and 198KB SRAMs. The ACNPU achieves 31.7 FPS and 124.4 FPS for x2 and x4 scales Full-HD generation, respectively, which attains 4.75 TOPS/W energy efficiency.

==> Makefile <==
TARGET=main
LATEX_BUILD_CMD=xelatex -synctex=1 -shell-escape -interaction=nonstopmode

default: build

build:
	$(LATEX_BUILD_CMD) $(TARGET).tex
	bibtex main.aux || true
	$(LATEX_BUILD_CMD) $(TARGET).tex
	$(LATEX_BUILD_CMD) $(TARGET).tex | grep 'Warning\|pages'
clean:
	rm -rf *.aux *.log *.gz *.bbl *.blg *.lof *.lot *.toc *.out

